ChildGAN: Large Scale Synthetic Child Facial Data Using Domain Adaptation in StyleGAN

In this research work, we proposed a novel ChildGAN, a pair of GAN networks for generating synthetic boys and girls facial data derived from StyleGAN2. ChildGAN is built by performing smooth domain transfer using transfer learning. It provides photo-realistic, high-quality data samples. A large-scale dataset is rendered with a variety of smart facial transformations: facial expressions, age progression, eye blink effects, head pose, skin and hair color variations, and variable lighting conditions. The dataset comprises more than 300k distinct data samples. Further, the uniqueness and characteristics of the rendered facial features are validated by running different computer vision application tests which include CNN-based child gender classifier, face localization and facial landmarks detection test, identity similarity evaluation using ArcFace, and lastly running eye detection and eye aspect ratio tests. The results demonstrate that synthetic child facial data of high quality offers an alternative to the cost and complexity of collecting a large-scale dataset from real children.

==> Tables/tab1.tex <==
\begin{table}[htb]
% \caption{OPEN-SOURCE CHILD DATASETS ATTRIBUTES}
% \label{tab1}
% \begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|l}
\cline{1-4}
DATASET & \begin{tabular}[c]{@{}c@{}}NUMBER\\ OF\\ SUBJECTS\end{tabular} & AGE & ATTRIBUTES &  \\ 
\cline{1-4}  \cline{1-4}
\begin{tabular}[c]{@{}c@{}}DuckEES\\ Database~\cite{DuckEES} {}{}\end{tabular} &
  NA &
  \begin{tabular}[c]{@{}c@{}}8\\ TO\\ 18\\ YEAR\\ OLDS\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1.The DuckEES\\  database contains \\  dynamic emotional\\  stimuli by children \\  and adolescent actors.\\ 2. It has a greater\\  representation of videos\\  thus comprising 142\\  posed videos which \\  is distributed relatively\\  homogeneously by\\  emotion.\\ 3.However, the\\  DuckEES dataset did\\  not include some of the\\  universal emotions such\\  that anger, contempt,\\  surprise.\end{tabular} &
   \\ \cline{1-4}
\begin{tabular}[c]{@{}c@{}}The\\ Child \\ Emotion\\  Facial \\ Expression\\  dataset~\cite{ChildEmotiondb} {}{}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}132 \\ CHILDREN\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}4\\ TO\\ 6\\ YEAR\\ OLDS\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1. A total of 29 hours \\  of video were recorded\\  in the studio for\\  capturing various child\\  facial expressions.\\ 2. The overall dataset\\  comes with eight\\  distinct facial\\  expressions which\\  includes contempt,\\  happiness, fear,\\  neutrality, disgust,\\  anger, surprise, and\\  sadness.\\ 3.The number of stimuli\\  of each emotion are as\\  follows: neutrality 87,\\  happiness 363, disgust\\  170, surprise 104, fear\\  153 (48 induced,\\  sadness 144, anger 157,\\  and contempt 183.\end{tabular} &
   \\ \cline{1-4}
\begin{tabular}[c]{@{}c@{}}The\\ Child \\ Affective\\  Facial \\ Expression\\  (CAFE) \\ dataset~\cite{CAFE} {}{}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}154 \\ CHILD \\ MODELS\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}2\\ TO\\ 8\\ YEAR\\ OLDS\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}1. Comprises data of 7\\  different facial\\  expressions which \\  includes sadness, \\  happiness, surprise, \\  anger, disgust, fear, and\\  neutral face.\\ 2. Not all children were\\  able to successfully\\  pose for all 7\\  expressions, so all\\  unsuccessful attempts\\  were eliminated from\\  the set.\\ 3. The result output data\\  consist of is 1192 total \\  photographs.\end{tabular} &
   \\ \cline{1-4} \cline{1-4}
\end{tabular}
}
% \end{center}
\caption{OPEN-SOURCE CHILD DATASETS ATTRIBUTES}
\label{tab1}
\end{table}

==> Tables/tab2.tex <==
% \begin{table}
% \begin{center}
% \begin{tabular}{|l|c|}
% \hline
% Method & Frobnability \\
% \hline\hline
% Theirs & Frumpy \\
% Yours & Frobbly \\
% Ours & Makes one's heart Frob\\
% \hline
% \end{tabular}
% \end{center}
% \caption{STYLEGAN2 HYPER-PARAMETER SELECTION}
% \end{table}

\begin{table}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|}
\hline 
S.no & Parameter                   & Value             \\ 
\hline \hline
  1    & Generator Learning Rate     & 0.002             \\
  2    & Discriminator Learning Rate & 0.002             \\
  3    & Batch Size                  & 128               \\
  4    & Generator Optimizer         & Adam              \\
  5    & Discriminator Optimizer     & Adam              \\
  6 & Generator Loss Function & \begin{tabular}[c]{@{}c@{}}Non-saturating logistic loss\\ with path length regularizer\end{tabular} \\
  7    & Discriminator Loss Function & R1 regularization \\
  8    & Metric                      & FID               \\
  9    & Mirror augment              & True              \\
 10   & Training epochs             & 500k              \\
 11   & Trunc psi                   & 0.6               \\ 
\hline 
\end{tabular}
}
\end{center}
\caption{StyleGAN2 hyper-parameter selection}
\label{tab2}
\end{table}

==> Tables/tab3.tex <==
\begin{table}[]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}ChildGAN \\ Data Category\end{tabular} & Number of Samples                                            & Image Resolution \\ 
\hline \hline
Boys images                                                       & 10k                                                          & 1024x1024        \\ \hline
Girls images                                                      & 10k                                                          & 1024x1024        \\ \hline
\begin{tabular}[c]{@{}c@{}}Facial Expressions\\ (Happy, Sad, \\ Surprise, and Angry)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Boys:48k \\ (12k/expression x 4)\\ Girls:48k\\ (12k/expression x 4)\end{tabular} &
  1024x1024 \\ 
  \hline
Eye blinking effect                                               & \begin{tabular}[c]{@{}c@{}}Boys:12k\\ Girls:12k\end{tabular} & 1024x1024        \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Skin Tone and \\ Hair Color \\ Variation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Boys:1k\\ Girls:1k\end{tabular} &
  1024x1024 \\ 
  \hline
\begin{tabular}[c]{@{}c@{}}Aging \\ Progression\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Boys:16k\\ Girls:16k\end{tabular} &
  1024x1024 \\ \hline
\begin{tabular}[c]{@{}c@{}}Head pose \\ Variation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Boys:30k\\ (16k yaw+14k pitch)\\ Girls:30k\\ (16k yaw+14k pitch)\end{tabular} &
  1024x1024 \\ \hline
Relighting                                                        & \begin{tabular}[c]{@{}c@{}}Boys:40k\\ Girls:40k\end{tabular} & 1024x1024        \\ \hline
\end{tabular}
}
\end{center}
\caption{Overall child synthetic dataset attributes.}
\label{tab3_old}
\end{table}

==> Tables/tab4.tex <==
\begin{table*}[htb]
\begin{tabular}{cccllllllll}
%\multicolumn{1}{l}{} &
%  \multicolumn{1}{l}{seed 5481} &
%  \multicolumn{1}{l}{seed 5483} &
%  seed 5505 &
%  seed5492 &
%  seed5469 &
%  seed5507 &
%  seed5477 &
%  seed5490 &
%  seed5474 &
%  seed5494 \\ 
\hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Subj 1} &
  \multicolumn{1}{c|}{Subj 2} &
  \multicolumn{1}{l|}{Subj 3} &
  \multicolumn{1}{l|}{Subj 4} &
  \multicolumn{1}{l|}{Subj 5} &
  \multicolumn{1}{l|}{Subj 6} &
  \multicolumn{1}{l|}{Subj 7} &
  \multicolumn{1}{l|}{Subj 8} &
  \multicolumn{1}{l|}{Subj 9} &
  \multicolumn{1}{l|}{Subj 10} \\ \hline
\multicolumn{1}{|c|}{Subj 1} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{0.3059} &
  \multicolumn{1}{l|}{0.2573} &
  \multicolumn{1}{l|}{0.3401} &
  \multicolumn{1}{l|}{0.2802} &
  \multicolumn{1}{l|}{0.4950} &
  \multicolumn{1}{l|}{0.3255} &
  \multicolumn{1}{l|}{0.4233} &
  \multicolumn{1}{l|}{0.3158} &
  \multicolumn{1}{l|}{0.4192} \\ \hline
\multicolumn{1}{|c|}{Subj 2} &
  \multicolumn{1}{c|}{0.3059} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{0.6590} &
  \multicolumn{1}{l|}{0.6965} &
  \multicolumn{1}{l|}{0.5293} &
  \multicolumn{1}{l|}{0.6223} &
  \multicolumn{1}{l|}{0.0774} &
  \multicolumn{1}{l|}{0.5898} &
  \multicolumn{1}{l|}{0.5245} &
  \multicolumn{1}{l|}{0.5106} \\ \hline
\multicolumn{1}{|c|}{Subj 3} &
  \multicolumn{1}{c|}{0.2573} &
  \multicolumn{1}{c|}{0.6590} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.6188} &
  \multicolumn{1}{l|}{0.5791} &
  \multicolumn{1}{l|}{0.7475} &
  \multicolumn{1}{l|}{0.2971} &
  \multicolumn{1}{l|}{0.6576} &
  \multicolumn{1}{l|}{0.7324} &
  \multicolumn{1}{l|}{0.5034} \\ \hline
\multicolumn{1}{|c|}{Subj 4} &
  \multicolumn{1}{c|}{0.3401} &
  \multicolumn{1}{c|}{0.6965} &
  \multicolumn{1}{l|}{0.6188} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.6471} &
  \multicolumn{1}{l|}{0.7113} &
  \multicolumn{1}{l|}{0.2343} &
  \multicolumn{1}{l|}{0.5758} &
  \multicolumn{1}{l|}{0.5393} &
  \multicolumn{1}{l|}{0.6640} \\ \hline
\multicolumn{1}{|c|}{Subj 5} &
  \multicolumn{1}{c|}{0.2802} &
  \multicolumn{1}{c|}{0.5293} &
  \multicolumn{1}{l|}{0.5791} &
  \multicolumn{1}{l|}{0.6471} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.5361} &
  \multicolumn{1}{l|}{0.3378} &
  \multicolumn{1}{l|}{0.5510} &
  \multicolumn{1}{l|}{0.5648} &
  \multicolumn{1}{l|}{0.5714} \\ \hline
\multicolumn{1}{|c|}{Subj 6} &
  \multicolumn{1}{c|}{0.4951} &
  \multicolumn{1}{c|}{0.6223} &
  \multicolumn{1}{l|}{0.7475} &
  \multicolumn{1}{l|}{0.7113} &
  \multicolumn{1}{l|}{0.5361} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.3618} &
  \multicolumn{1}{l|}{0.7413} &
  \multicolumn{1}{l|}{0.5970} &
  \multicolumn{1}{l|}{0.6636} \\ \hline
\multicolumn{1}{|c|}{Subj 7} &
  \multicolumn{1}{c|}{0.3255} &
  \multicolumn{1}{c|}{0.0774} &
  \multicolumn{1}{l|}{0.2971} &
  \multicolumn{1}{l|}{0.2342} &
  \multicolumn{1}{l|}{0.3378} &
  \multicolumn{1}{l|}{0.3618} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.4421} &
  \multicolumn{1}{l|}{0.4140} &
  \multicolumn{1}{l|}{0.2997} \\ \hline
\multicolumn{1}{|c|}{Subj 8} &
  \multicolumn{1}{c|}{0.4233} &
  \multicolumn{1}{c|}{0.5898} &
  \multicolumn{1}{l|}{0.6575} &
  \multicolumn{1}{l|}{0.5758} &
  \multicolumn{1}{l|}{0.5509} &
  \multicolumn{1}{l|}{0.7413} &
  \multicolumn{1}{l|}{0.4421} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.5801} &
  \multicolumn{1}{l|}{0.4302} \\ \hline
\multicolumn{1}{|l|}{Subj 9} &
  \multicolumn{1}{l|}{0.3158} &
  \multicolumn{1}{l|}{0.5245} &
  \multicolumn{1}{l|}{0.7324} &
  \multicolumn{1}{l|}{0.5393} &
  \multicolumn{1}{l|}{0.5648} &
  \multicolumn{1}{l|}{0.5970} &
  \multicolumn{1}{l|}{0.4140} &
  \multicolumn{1}{l|}{0.5801} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.4601} \\ \hline
\multicolumn{1}{|l|}{Subj 10} &
  \multicolumn{1}{l|}{0.4192} &
  \multicolumn{1}{l|}{0.5106} &
  \multicolumn{1}{l|}{0.5034} &
  \multicolumn{1}{l|}{0.6640} &
  \multicolumn{1}{l|}{0.5714} &
  \multicolumn{1}{l|}{0.6636} &
  \multicolumn{1}{l|}{0.2998} &
  \multicolumn{1}{l|}{0.4302} &
  \multicolumn{1}{l|}{0.4607} &
  \multicolumn{1}{l|}{} \\ \hline
\end{tabular}
\caption{Identity similarity scores using ArcFace for girls}
\label{tab4-girls-old}
\end{table*}

\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 %& seed 9971 & seed 9988 & seed 9978 & seed 9970 & seed 9997 & seed 9974 & seed 9952 & seed9960 & seed9958 & seed9981 \\ \hline
        & Subj 1 & Subj 2 & Subj 3 & Subj 4 & Subj 5 & Subj 6 & Subj 7 & Subj 8 & Subj 9 & Subj 10 \\ \hline
Subj 1  &        & 0.7034 & 0.3473 & 0.6283 & 0.6092 & 0.6693 & 0.3613 & 0.6690 & 0.5897 & 0.6972  \\ \hline
Subj 2  & 0.7034 &        & 0.3616 & 0.7845 & 0.5406 & 0.4923 & 0.3594 & 0.6650 & 0.3587 & 0.6283  \\ \hline
Subj 3  & 0.3473 & 0.3616 &        & 0.3126 & 0.3254 & 0.5024 & 0.1651 & 0.4799 & 0.2848 & 0.4276  \\ \hline
Subj 4  & 0.6283 & 0.7845 & 0.3126 &        & 0.6222 & 0.5543 & 0.3886 & 0.6542 & 0.3750 & 0.6841  \\ \hline
Subj 5  & 0.6092 & 0.5406 & 0.3254 & 0.6222 &        & 0.6362 & 0.4768 & 0.4541 & 0.3038 & 0.5852  \\ \hline
Subj 6  & 0.6693 & 0.4923 & 0.5024 & 0.5543 & 0.6362 &        & 0.3315 & 0.6617 & 0.4835 & 0.7464  \\ \hline
Subj 7  & 0.3613 & 0.3594 & 0.1651 & 0.3886 & 0.4768 & 0.3315 &        & 0.2844 & 0.1764 & 0.3510  \\ \hline
Subj 8  & 0.6690 & 0.6650 & 0.4799 & 0.6542 & 0.4541 & 0.6617 & 0.2844 &        & 0.5137 & 0.7423  \\ \hline
Subj 9  & 0.5897 & 0.3587 & 0.2818 & 0.3750 & 0.3038 & 0.4835 & 0.1764 & 0.5137 &        & 0.5965  \\ \hline
Subj 10 & 0.6972 & 0.6283 & 0.4276 & 0.6841 & 0.5852 & 0.7464 & 0.3510 & 0.7423 & 0.5965 &         \\ \hline
\end{tabular}
\caption{Identity similarity scores using ArcFace for boys}
\label{tab4-boys-old}
\end{table*}

==> Tables/tab4test.tex <==
\begin{table*}[htb]
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cccllllllll}
% \multicolumn{1}{l}{} &
%  \multicolumn{1}{l}{seed 5481} &
%  \multicolumn{1}{l}{seed 5483} &
%  seed 5505 &
%  seed5492 &
%  seed5469 &
%  seed5507 &
%  seed5477 &
%  seed5490 &
%  seed5474 &
%  seed5494 \\ 
\hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Subj 1 } &
  \multicolumn{1}{c|}{Subj 2 } &
  \multicolumn{1}{l|}{Subj 3 } &
  \multicolumn{1}{l|}{Subj 4 } &
  \multicolumn{1}{l|}{Subj 5 } &
  \multicolumn{1}{l|}{Subj 6 } &
  \multicolumn{1}{l|}{Subj 7 } &
  \multicolumn{1}{l|}{Subj 8 } &
  \multicolumn{1}{l|}{Subj 9 } &
  \multicolumn{1}{l|}{Subj 10} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5481.png}}\\ Subj 1\end{tabular}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{0.3059} &
  \multicolumn{1}{l|}{0.2573} &
  \multicolumn{1}{l|}{0.3401} &
  \multicolumn{1}{l|}{0.2802} &
  \multicolumn{1}{l|}{0.4950} &
  \multicolumn{1}{l|}{0.3255} &
  \multicolumn{1}{l|}{0.4233} &
  \multicolumn{1}{l|}{0.3158} &
  \multicolumn{1}{l|}{0.4192} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5483.png}}\\ Subj 2\end{tabular}} &
  \multicolumn{1}{c|}{0.3059} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{0.6590} &
  \multicolumn{1}{l|}{0.6965} &
  \multicolumn{1}{l|}{0.5293} &
  \multicolumn{1}{l|}{0.6223} &
  \multicolumn{1}{l|}{0.0774} &
  \multicolumn{1}{l|}{0.5898} &
  \multicolumn{1}{l|}{0.5245} &
  \multicolumn{1}{l|}{0.5106} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5505.png}}\\ Subj 3\end{tabular}} &
  \multicolumn{1}{c|}{0.2573} &
  \multicolumn{1}{c|}{0.6590} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.6188} &
  \multicolumn{1}{l|}{0.5791} &
  \multicolumn{1}{l|}{0.7475} &
  \multicolumn{1}{l|}{0.2971} &
  \multicolumn{1}{l|}{0.6576} &
  \multicolumn{1}{l|}{0.7324} &
  \multicolumn{1}{l|}{0.5034} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5492.png}}\\ Subj 4\end{tabular}} &
  \multicolumn{1}{c|}{0.3401} &
  \multicolumn{1}{c|}{0.6965} &
  \multicolumn{1}{l|}{0.6188} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.6471} &
  \multicolumn{1}{l|}{0.7113} &
  \multicolumn{1}{l|}{0.2343} &
  \multicolumn{1}{l|}{0.5758} &
  \multicolumn{1}{l|}{0.5393} &
  \multicolumn{1}{l|}{0.6640} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5469.png}}\\ Subj 5\end{tabular}} &
  \multicolumn{1}{c|}{0.2802} &
  \multicolumn{1}{c|}{0.5293} &
  \multicolumn{1}{l|}{0.5791} &
  \multicolumn{1}{l|}{0.6471} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.5361} &
  \multicolumn{1}{l|}{0.3378} &
  \multicolumn{1}{l|}{0.5510} &
  \multicolumn{1}{l|}{0.5648} &
  \multicolumn{1}{l|}{0.5714} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5507.png}}\\ Subj 6\end{tabular}} &
  \multicolumn{1}{c|}{0.4951} &
  \multicolumn{1}{c|}{0.6223} &
  \multicolumn{1}{l|}{0.7475} &
  \multicolumn{1}{l|}{0.7113} &
  \multicolumn{1}{l|}{0.5361} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.3618} &
  \multicolumn{1}{l|}{0.7413} &
  \multicolumn{1}{l|}{0.5970} &
  \multicolumn{1}{l|}{0.6636} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5477.png}}\\ Subj 7\end{tabular}} &
  \multicolumn{1}{c|}{0.3255} &
  \multicolumn{1}{c|}{0.0774} &
  \multicolumn{1}{l|}{0.2971} &
  \multicolumn{1}{l|}{0.2342} &
  \multicolumn{1}{l|}{0.3378} &
  \multicolumn{1}{l|}{0.3618} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.4421} &
  \multicolumn{1}{l|}{0.4140} &
  \multicolumn{1}{l|}{0.2997} \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5490.png}}\\ Subj 8\end{tabular}} &
  \multicolumn{1}{c|}{0.4233} &
  \multicolumn{1}{c|}{0.5898} &
  \multicolumn{1}{l|}{0.6575} &
  \multicolumn{1}{l|}{0.5758} &
  \multicolumn{1}{l|}{0.5509} &
  \multicolumn{1}{l|}{0.7413} &
  \multicolumn{1}{l|}{0.4421} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.5801} &
  \multicolumn{1}{l|}{0.4302} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5474.png}}\\ Subj 9\end{tabular}} &
  \multicolumn{1}{l|}{0.3158} &
  \multicolumn{1}{l|}{0.5245} &
  \multicolumn{1}{l|}{0.7324} &
  \multicolumn{1}{l|}{0.5393} &
  \multicolumn{1}{l|}{0.5648} &
  \multicolumn{1}{l|}{0.5970} &
  \multicolumn{1}{l|}{0.4140} &
  \multicolumn{1}{l|}{0.5801} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{0.4601} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/girl_samples/seed5494.png}}\\ Subj 10\end{tabular}} &
  \multicolumn{1}{l|}{0.4192} &
  \multicolumn{1}{l|}{0.5106} &
  \multicolumn{1}{l|}{0.5034} &
  \multicolumn{1}{l|}{0.6640} &
  \multicolumn{1}{l|}{0.5714} &
  \multicolumn{1}{l|}{0.6636} &
  \multicolumn{1}{l|}{0.2998} &
  \multicolumn{1}{l|}{0.4302} &
  \multicolumn{1}{l|}{0.4607} &
  \multicolumn{1}{l|}{} \\ \hline
\end{tabular}
}
\end{center}
\caption{Identity similarity scores using ArcFace for girls}
\label{tab4-girls}
\end{table*}


\begin{table*}[htb]
\begin{center}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
% & seed 9971 & seed 9988 & seed 9978 & seed 9970 & seed 9997 & seed 9974 & seed 9952 & seed9960 & seed9958 & seed9981 \\ \hline
& Subj 1 & Subj 2 & Subj 3 & Subj 4 & Subj 5 & Subj 6 & Subj 7 & Subj 8 & Subj 9 & Subj 10 \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9971.png}}\\ Subj 1\end{tabular}  &        & 0.7034 & 0.3473 & 0.6283 & 0.6092 & 0.6693 & 0.3613 & 0.6690 & 0.5897 & 0.6972  \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9988.png}}\\ Subj 2\end{tabular}  & 0.7034 &        & 0.3616 & 0.7845 & 0.5406 & 0.4923 & 0.3594 & 0.6650 & 0.3587 & 0.6283  \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9978.png}}\\ Subj 3\end{tabular}  & 0.3473 & 0.3616 &        & 0.3126 & 0.3254 & 0.5024 & 0.1651 & 0.4799 & 0.2848 & 0.4276  \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9970.png}}\\ Subj 4\end{tabular}  & 0.6283 & 0.7845 & 0.3126 &        & 0.6222 & 0.5543 & 0.3886 & 0.6542 & 0.3750 & 0.6841  \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9997.png}}\\ Subj 5\end{tabular}  & 0.6092 & 0.5406 & 0.3254 & 0.6222 &        & 0.6362 & 0.4768 & 0.4541 & 0.3038 & 0.5852  \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9974.png}}\\ Subj 6\end{tabular}  & 0.6693 & 0.4923 & 0.5024 & 0.5543 & 0.6362 &        & 0.3315 & 0.6617 & 0.4835 & 0.7464  \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9952.png}}\\ Subj 7\end{tabular}  & 0.3613 & 0.3594 & 0.1651 & 0.3886 & 0.4768 & 0.3315 &        & 0.2844 & 0.1764 & 0.3510  \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9960.png}}\\ Subj 8\end{tabular}  & 0.6690 & 0.6650 & 0.4799 & 0.6542 & 0.4541 & 0.6617 & 0.2844 &        & 0.5137 & 0.7423  \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9958.png}}\\ Subj 9\end{tabular}  & 0.5897 & 0.3587 & 0.2818 & 0.3750 & 0.3038 & 0.4835 & 0.1764 & 0.5137 &        & 0.5965  \\ \hline
\begin{tabular}[c]{@{}c@{}} \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth]{iccv2023AuthorKit/Figures/boy_samples/seed9981.png}}\\ Subj 10\end{tabular} & 0.6972 & 0.6283 & 0.4276 & 0.6841 & 0.5852 & 0.7464 & 0.3510 & 0.7423 & 0.5965 &         \\ \hline
\end{tabular}
}
\end{center}
\caption{Identity similarity scores using ArcFace for boys}
\label{tab4-boys}
\end{table*}
